A Dual-Beam Method-of-Images 3D Searchlight BSSRDF

We present a novel BSSRDF for rendering translucent materials. Angular effects lacking in previous BSSRDF models are incorporated by using a dual-beam formulation. We employ a Placzek's Lemma interpretation of the method of images and discard diffusion theory. Instead, we derive a plane-parallel transformation of the BSSRDF to form the associated BRDF and optimize the image confiurations such that the BRDF is close to the known analytic solutions for the associated albedo problem. This ensures reciprocity, accurate colors, and provides an automatic level-of-detail transition for translucent objects that appear at various distances in an image. Despite optimizing the subsurface fluence in a plane-parallel setting, we find that this also leads to fairly accurate fluence distributions throughout the volume in the original 3D searchlight problem. Our method-of-images modifications can also improve the accuracy of previous BSSRDFs.

==> beamtobeam.tex <==
\section{Beam to beam evaluation}

    We require evaluating the integrals of an exponential isotropic source function (the source beam) for each location on the exitant exponential exitance path.

    \subsection{Once-collided Flux Kernel}
    The density of light in an infinite volume due to an extended source is a sum of two terms (Equation~\ref{grosjeanphi}).  The exitant path-integral of the once-collided-flux involves the kernel:
    \begin{equation}\label{KOCF}
        K_{OCF}(r) = \frac{1}{4 \pi r^2} \exp(-\mu_t' r).
    \end{equation}
    For any fixed point on one of the lines of integration the integration of the other variable is efficiently computed using a series expansion due to Rief et al.~\shortcite{rief84} which is efficiently computed using a recurrence relation:
    \begin{align}
        B_0 &= \left( \frac{\pi}{2} - \arcsin \left[ \frac{h}{(L^2+h^2)^{1/2}}\right] \right) \frac{1}{h} \\
        B_1 &= -(\mu_t') \log \left[ \frac{L+(L^2+h^2)^{1/2}}{h} \right] \\
        B_2 &= \frac{ (\mu_t')^2}{2} L \\
        B_n &= (-1)^n \frac{(\mu_t')^n L}{(n-1)n!} (L^2+h^2)^{(n-2)/2} + \frac{(n-1) (\mu_t')^2 h^2}{(n-1)^2 n} B_{n-2}
    \end{align}

    \subsection{Modified Diffusion Kernel}
    The multiply-scattered light involves the modified diffusion kernel:
    \begin{equation}\label{Kdiffusion}
        K_D(r) = \frac{1}{4 \pi} \frac{3 \mu_s' \mu_t'}{2 \mu_a + \mu_s'} \frac{\e^{- \sqrt{\frac{\mu_a}{D}} r}}{r}.
    \end{equation}



